A Moving-Horizon Hybrid Stochastic Game for Secure Control of Cyber-Physical Systems

In this paper, we establish a zero-sum, hybrid state stochastic game model for designing defense policies for cyber-physical systems against different types of attacks. With the increasingly integrated properties of cyber-physical systems (CPS) today, security is a challenge for critical infrastructures. Though resilient control and detecting techniques for a specific model of attack have been proposed, to analyze and design detection and defense mechanisms against multiple types of attacks for CPSs requires new system frameworks. Besides security, other requirements such as optimal control cost also need to be considered. The hybrid game model we propose in this work contains physical states that are described by the system dynamics, and a cyber state that represents the detection mode of the system composed by a set of subsystems. A strategy means selecting a subsystem by combining one controller, one estimator and one detector among a finite set of candidate components at each state. Based on the game model, we propose a suboptimal value iteration algorithm for a finite horizon game, and prove that the algorithm results an upper bound for the value of the finite horizon game. A moving-horizon approach is also developed in order to provide a scalable and real-time computation of the switching strategies. Both algorithms aims at obtaining a saddle-point equilibrium policy for balancing the system's security overhead and control cost. The paper illustrates these concepts using numerical examples, and we compare the results with previously system designs that only equipped with one type of controller.

==> abstract.tex <==
\begin{abstract}
\label{abstract}
 In this paper, we establish a zero-sum, hybrid state stochastic game model for designing defense policies for cyber-physical systems against different types of attacks. With the increasingly integrated properties of cyber-physical systems (CPS) today, security is a challenge for critical infrastructures. Though resilient control and detecting techniques for a  specific model of attack have been proposed, to analyze and design detection and defense mechanisms against multiple types of attacks for CPSs requires new system frameworks. Besides security, other requirements such as optimal control cost also need to be considered. The hybrid game model we propose in this work contains physical states that are described by the system dynamics, and a cyber state that represents the detection mode of the system composed by a set of subsystems. A strategy means selecting a subsystem by combining one controller, one estimator and one detector among a finite set of candidate components at each state. Based on the game model, we propose a suboptimal value iteration algorithm for a finite horizon game, and prove that the algorithm results an upper bound for the value of the finite horizon game. A moving-horizon approach is also developed in order to provide a scalable and real-time computation of the switching strategies. Both algorithms aims at obtaining a saddle-point equilibrium policy for balancing the system's security overhead and control cost. 
%This approach leads to a real-time algorithm that yields a sequence of Nash equilibrium strategies which can be shown to converge. 
The paper illustrates these concepts using numerical examples, and we compare the results with previously system designs that only equipped with one type of controller. 


\iffalse
In the hybrid model, a system is equipped with a given finite set of controllers/estimators/detectors, and switching mechanisms can be used to select a subsystem--a combination of one controller, one estimator and one detector at each time step. 
\fi

\iffalse
The moving-horizon approach uses a moving window to select a sequence of physical state information, and computes a stationary saddle-point equilibrium strategies with the state being a joint cyber and physical state. 
\fi
%Game parameters are quantified with knowledge of the system dynamics and attack models.
%The game state describes both a sequence of physical dynamics and a piecewise constant detection mode of the system, such that the state transition is Markov and the game moves the horizon of system information at every stage.
%developed, for minimizing the expected current stage payoff when looking ahead into ensuing stages, and reducing the computation overhead of previous proposed suboptimal algorithm. The convergence property of the algorithm is shown.%, followed by the stability condition of the system. 
%Using a linear system with control-cost optimal (but nonsecure) and secure (but cost-suboptimal) controllers in presence of replay attacks as an example, 
 
\end{abstract}

==> algorithm_1.tex <==
%\section{Algorithms for Finite and Infinite Horion Game}
\section{Suboptimal Algorithm for Finite Horizon Game}
\label{sec:algorithm_finite}

Based on the game formulation, in this section we discuss the existence of an optimal finite horizon solution for the system, and present an algorithm to compute a suboptimal strategy for the system. 
In this section, we propose a moving-horizon algorithm to compute the saddle-point equilibrium strategy of the hybrid stochastic game.  Illustrated in Fig. 2, a time window of size $T$ is used, and an equilibrium strategy is computed at each stage $k$ by looking back $T$ stages of the physical state $x_{[k-T, k]}$ and its associated cyber state $\delta_l$. Detailed process of moving the horizon to obtain predicted future stage information is described in Subsection~\ref{move_horizon}.  Algorithm~\ref{finite_new} is developed based on this concept, and provides a scalable and real-time computation process, which allows us to analyze the convergence property of the strategies of the hybrid stochastic game in Subsection~\ref{converge}. 

\subsection{A Moving-Horizon Approach for Hybrid Stochastic Game}
\label{sec:algorithm}
%Based on the game formulation, in this section, we define an objective function and the optimal strategy for both players, and 
In this section, we propose a moving-horizon algorithm to compute the saddle-point equilibrium strategy of the hybrid stochastic game.  Illustrated in Fig. 2, a time window of size $T$ is used, and an equilibrium strategy is computed at each stage $k$ by looking back $T$ stages of the physical state $x_{[k-T, k]}$ and its associated cyber state $\delta_l$. Detailed process of moving the horizon to obtain predicted future stage information is described in Subsection~\ref{move_horizon}.  Algorithm~\ref{finite_new} is developed based on this concept, and provides a scalable and real-time computation process, which allows us to analyze the convergence property of the strategies of the hybrid stochastic game in Subsection~\ref{converge}. 
%and the stability property of the system.
\subsubsection{A Moving-Horizon Algorithm for Game Strategies}
\label{move_horizon}
The saddle-point equilibrium strategy and the value of the moving-horizon game at each stage involves solving finite zero-sum matrix games. 
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this paper, we consider an objective function that reflects the payoff of the game at the current stage $k$, and also the expected payoff from the future stage. By looking one stage ahead of the game state at $k$, predicting the physical dynamics $\mathbf{x}_{k+1}$ given any action pair, we move the information horizon to stage $k+1$ and obtain future expectation for computing the strategies at stage $k$. The moving horizon process is illustrated as Figure~\ref{sg}. 
%We obtain a zero-sum game at stage $k$ to solve as in Definition~\ref{zero_sum}, 
Detailed process to construct the payoff matrix of a zero-sum game for stage $k$ is described, and Algorithm~\ref{finite_new} presents the complete equilibrium computation process of the hybrid stochastic game.
    
\iffalse When we calculate the expected value of the game at stage $k+1$, treat it as a termination. \fi
Given any action pair $(a_{ik},u_{jk})$ at stage $k$, we first update the state space form of the system dynamics $\mathbf{x}_{k+1}$ based on $\mathbf{x}_{[k-T,k]}$ as~\eqref{dynamicgame}. We view $\mathbf{x}_{k+1}$ as a function of $(\mathbf{x}_{[k-T, k]}, a_{ik},u_{jk})$, the immediate payoff function $\tilde{r}_{k+1} (s_{(k+1)h})$ (for stage $k+1$) defined as~\eqref{payoff} is a function of $s_{(k+1)h}=(\mathbf{x}_{[k-T+1,k+1]}, \delta_h)$, thus $r_{k+1}$ is a function of $(\mathbf{x}_{[k-T, k]}, a_{ik},u_{jk}, \delta_h)$, as shown in the following equation~\eqref{prev}.
Then, we compute the value of the matrix game at stage $k+1$, for every $r_{k+1}(\mathbf{x}_{[k-T,k]},a_{ik},u_{jk},\delta_h)$, $h=1,2,3,$ $i\in \{1,\cdots, M\}, j \in \{1,\cdots, N\}$ as~\eqref{prev}:
%$v^{ij}_{k+1}(s_{(k+1)h}) \leftarrow \pi (r_{k+1}(s_{(k+1)h}))$;\\
\begin{align}
v^{ij}_{k+1}(x_{[x-T,k]},\delta_h)= \min\limits_{\mathbf{g}}\max\limits_{\mathbf{f}}(r_{k+1}(\mathbf{x}_{[k-T,k]},a_{ik},u_{jk},\delta_h))
\label{prev}
\end{align}

With the predicted value from the next stage, define the auxiliary matrix for stage $k$ as:
\footnotesize
\begin{align}
\begin{split}
Q_{k}(s_{kl})=r_{k}(s_{kl})
                         +\sum_{s_h\in S} \tilde{P}_{k}( s_{(k+1)h} |s_{kl})\cdot v_{k+1}(x_{[k-T,k]},\delta_h),
\end{split}
\label{Q_k}
\end{align}
\normalsize
where the matrix $v^{ij}_{k+1}(x_{[x-T,k]},\delta_h)$ is defined by~\eqref{prev}, and it is the element of the $i$th row, $j$th column of the matrix $$v_{k+1}(x_{[k-T,k]},\delta_h) \in \mathbb{R}^{M \times N}.$$ %Then the optimal solution for stage $k$ of the real time Algorithm~\ref{finite_new}.
The dot products between two matrices $\tilde{P}_{k}( s_{(k+1)h} |s_{kl})$, $v_{k+1}(x_{[k-T,k]},\delta_h)$ is an element wise product of two elements at the same position of the two matrices.
\iffalse we first predict the payoff matrix of stage $k+1$ for every action pair $(a_{ik}, u_{jk})$, which is denoted as $r_{k+1}(\mathbf{x}_{[k-T,k]},a_{ik},u_{jk},\delta_h), h=1,2,3$. For getting a payoff matrix at state $s_{kl}$, \fi

The value and stationary equilibrium strategies that Algorithm~\ref{finite_new} calculates at each stage $k$ is defined as following:
\begin{definition}
Given $s_{kl}$, $v_{k+1}(x_{[k-T,k]},\delta_h)$ as~\eqref{prev}, and auxiliary matrix $Q_{k}(s_{kl})$ as~\eqref{Q_k}, the value and equilibrium strategies at $k$ are defined as the following equation: 
\begin{align}
v(s_{kl})= \min\limits_{\mathbf{g}_k(s_{kl})}\max\limits_{\mathbf{f}_k(s_{kl})} \mathbf{f}_k(s_{kl})^T Q_{k}(s_{kl}) \mathbf{g}_k(s_{kl}).
\label{v_k}
\end{align}
Where we treat the auxiliary matrix $Q_{k}(s_{kl})$ as the payoff matrix of a zero-sum game of stage $k$. 
%The value and equilibrium strategies of the matrix game $Q_{k}(s_{kl})$ consist with the meaning of value and equilibrium strategies in Definition~\ref{zero_sum}.
\end{definition}

At each stage $k$, we repeat calculating $Q_{k}(s_{kl})$ and the corresponding value and equilibrium strategies, then update the system dynamics by the strategies for computation of next stage. The complete process is summarized as Algorithm~\ref{finite_new}. 
%\newtheorem{algorithm}{Algorithm}
\begin{algorithm}
%\label{finite_new}
\caption{\textbf{: Moving-Horizon Algorithm for A Hybrid Stochastic Game}}
%\begin{algorithmic}
\textbf{Input}: System model parameters and game parameters.
\\\textbf{Initialization}: $\hat{\mathbf{x}}_{1|0}, \mathbf{x}_1$.
\\\textbf{Iteration}: For $k=T, \cdots, K+T-1$,                                                                                 
 $s_{kl}=(x_{[k-T,k]},\delta_l),$  $l=1,2,3$:  
get  the auxiliary matrix~\eqref{Q_k} for stage k;
%\[Q_{k}(s_{kl}) = r_{k}(s_{kl})+\sum_{s_h\in S} \tilde{P}_{k}( s_{(k+1)h} |s_{kl})\cdot v_{k+1}(x_{[k-T,k]},\delta_h),\]
compute the value and equilibrium strategies of every matrix game:\\
$v(s_{kl})= \min\limits_{\mathbf{g}(s_{kl})}\max\limits_{\mathbf{f}(s_{kl})} \mathbf{f}(s_{kl})^T Q_{k}(s_{kl}) \mathbf{g}(s_{kl})$,\\
$\mathbf{f}_k^{*}(s_{kl})=\arg \max\limits_{\mathbf{f}_k(s_{kl})}\mathbf{f}_k(s_{kl})^T Q_{k}(s_{kl} )\mathbf{g}_k^*(s_{kl})$, \\
$\mathbf{g}_k^{*}(s_{kl})=\arg \min\limits_{\mathbf{g}_k(s_{kl})} [\mathbf{f}_k^{*}(s_{kl})]^T Q_{k}(s_{kl}) \mathbf{g}_k(s_{kl})$.\\
Update the system dynamics with strategies $\mathbf{f}_k^{*}(s_{kl}),\mathbf{g}_k^{*}(s_{kl}),$ $l=1,2,3$ as described in~\ref{dynamicgame} for the next stage.
\\\textbf{Return}: the concatenation of strategies for both players $\mathbf{f}=\{f_k^{*}(s_{kl})\},\mathbf{g}=\{\mathbf{g}^*_k(s_{kl})\}$ and the value sequence $v_{k}(s_{kl}),k=1,\cdots, K, l=1,2,3$.
\label{finite_new}
\end{algorithm}
To get the total payoff till stage $k$ by Algorithm~\ref{finite_new}, we plug in the strategies $\mathbf{f}, \mathbf{g}$ to the system dynamics and calculate the sum of payoff for all stages.%as Definition~\ref{R_K} for $k$ stages.
\iffalse
Miao~\textit{et al.} designed a suboptimal value iterative algorithm and proved a value upper bound for the stochastic game in~\cite{cdc_replay}. The suboptimal algorithm is exponential time with respect to K, since before value iteration, it computes the extreme points for the payoff and state transition probability set--the number of extreme points increases exponentially with the stage number $K$.  When running offline, this algorithm works well in the sense that total payoff of $K$ stages  are considered for the game.   
\fi
\begin{remark}
It is worth noting that~Algorithm~\ref{finite_new} reduces the computation overhead for the hybrid stochastic game, since it looks one stage ahead with a moving-horizon information window. The complexity of Algorithm~\eqref{finite_new} is $O(K)$. For a large total stage number of the hybrid stochastic game $\tilde{T}$, it is necessary to examine the strategy trend of Algorithm~\ref{finite_new}, such as convergence property. As a contrast, the suboptimal algorithm in~\cite{cdc_replay} takes the total expected payoff as an objective function. The complexity of suboptimal algorithm is exponential with stage number $K$, because the algorithm looks $K$ stages ahead at once and compute a robust game for every iteration. The advantage of suboptimal algorithm in~\cite{cdc_replay} is to provide an upper bound of the total finite cost. However, for a large $\tilde{T}$,  the suboptimal algorithm in~\cite{cdc_replay} is computationally expensive. Numerical comparisons are shown in Section~\ref{sec:simulation}.
\iffalse
To get a suboptimal total payoff of time $\tilde{T}$ faster, we can view this as a $K$ stage game, and at each stage the physical dynamics run $[\tilde{T}/K]$ steps as~\eqref{eq:xu}. The average payoff and state transition probability in the $[\tilde{T}/K]$ discrete time slots are the payoff and state transition probability of one game stage.  
In particular, when we consider the average of infinite horizon time $\tilde{T}$, the game can reduce to a stationary stochastic game. For example, with the infinite time average LQG cost as the payoff function, and the average detection rate, false alarm trigger rate as the state transition probability, we actually reach the optimal strategy of a stationary stochastic game.  
\fi

\end{remark}
\subsubsection{Convergence Analysis of the Algorithm}
\label{coverge}
Given the sets of models for each component of the subsystems and attacks, the system dynamics are defined by a sequence of action pairs $(a_{ik},u_{jk}), k \in \{k+T, \cdots, K+T\}$ randomly chosen by the attacker and the system. 
Then, the system dynamics with the stochastic game strategies (for the system and the attacker) are equivalent with a switched system -- the system model randomly switches among $N$ subsystems, according to strategies $\mathbf{f}_k(s_{kl})$. %[\mathbf{g}_k(s_{kl})]^T$. 
The following theorem shows the existence condition of convergent strategies when $k\to \infty$. 
When there exists such strategies, the switched system can be described as a Markov jump system, since the state transition probability also converges. 
%\newtheorem{theorem}{Theorem}
\begin{proposition}
%The nonstationary stochastic game has a stationary strategy
The strategy sequences $\mathbf{f}_k^*(s_{kl})$, $\mathbf{g}_k^*(s_{kl})$ of the stochastic game converge to $\mathfrak{f}^l,\mathfrak{g}^l $, $l=1,2,3$, i.e.,
\begin{align*}
\mathfrak{f}^l=\lim\limits_{k\to\infty}\mathbf{f}_k^*(s_{kl}), \mathfrak{g}^l=\lim\limits_{k\to\infty}\mathbf{g}_k^*(s_{kl}), l=1,2,3,
\end{align*}
if updating system dynamics at stage $k+1$ by ($\mathfrak{f}^l,\mathfrak{g}^l$) results in:
\begin{align}
\lim \limits_{k \to \infty} Q_{k}(s_{kl})=\lim \limits_{k \to \infty} Q_{k}(s_{(k+1)l}), l=1,2,3.
\label{station}
\end{align}
%\end{equation}
\end{proposition}
\begin{proof}
According to Algorithm~\ref{finite_new}, the strategies $\mathbf{f}^*_k(s_{kl})$, $\mathbf{g}^*_k(s_{kl}),l=1,2,3$ are the saddle-point equilibrium strategies for the payoff matrices $Q_{k}(s_{kl}),l=1,2,3$. 
\iffalse After calculating the strategies at stage $k$, the next step of the Algorithm~\ref{finite_new} is updating the system dynamics, and then getting the auxiliary matrices $Q_{k}(s_{(k+1)l}),l=1,2,3$ for stage $k+1$. 
The saddle-point equilibrium strategies at stage $k+1$ are decided by $Q_{k}(s_{(k+1)l}),l=1,2,3$. 
Thus, if updating the system dynamics for the auxiliary matrix $Q_{k}(s_{kl})$ and at each mode $Q_{k}(s_{kl})$  converges with an optimal strategy for both players, \fi
Thus, if~\eqref{station} holds, the auxiliary matrix $Q_{k}(s_{kl})$ converges, and we get convergent strategies for both players. 
%The nonstationary stochastic game then converges to a stationary one, the switching probability of the system then does not change with $k$.%
%turns to a homogeneous Markov jump system--the switching probability distribution is determined by 
%%
%$\tilde{P}_k(s_{(k+1)h}|s_{kl})$.
\end{proof}
\iffalse
\begin{proposition}
If the control input $\gamma(a_{ik}, u_{jk})=L_j\hat{\mathbf{x}}_{t}, t\in[k-T, k]$ for any action pair $(a_{ik}, u_{jk})$, then the system is not asymptotically stable when the strategy sequences $\mathbf{f}_k^*(s_{kl})$, $\mathbf{g}_k^*(s_{kl})$ of the stochastic game are not convergent.
\end{proposition}
%\begin{proof}

Sketch of the proof: 
When the system is asymptotically stable, $\lim_{k\to\infty}\mathbf{Ex}_k=0$, by the definition of immediate payoff function~\eqref{payoff}, we gave $$
After calculating the strategies at stage $k$, the next step of the Algorithm~\ref{finite_new} is updating the system dynamics, and then getting the auxiliary matrices $Q_{k}(s_{(k+1)l}),l=1,2,3$ for stage $k+1$. 
%\end{proof}
\fi
\begin{remark}
When the strategy sequences of both players converge, the switched system dynamics converge to a discrete-time Markov jump linear system (with delays when the attacker's strategies include replay attacks), then we analyze the stability properties of the system based on conclusions of previous work~\cite{delay_mlj}.
\end{remark}
%Assume that every subsystem is mean square exponentially stable (i.e., attacks can increase the cost of every subsystem, but can not destabilize the system), 
 %\cite{dtls_mj},~\cite{dtass_mj}. 
%When the strategy sequences do not converge, condition of system stability is considered as future work. 

It is possible that some subsystems $u_{jk}, j \in \{1,\cdots, N\}$  are unstable under specific types of attacks.
When this is the case, the system switches among stable and unstable subsystems. Stability properties of continuous time linear switched systems including unstable modes are analyzed in~\cite{switch_unstable}. To guarantee exponential stability, the total activation time of unstable subsystems need to be relatively small compared with that of stable subsystems. Given the stochastic game strategy, we get the switched dynamic process of the system under different types of attacks, and check whether stability conditions are violated. 
More analysis of system stability conditions based on the moving horizon stochastic game framework will be an avenue of future work.
%For the discrete time switched system switches among stable and unstable subsystems, where the transition probability is determined by the game strategy, the stability property still needs future analysis.
\iffalse the system is still Markov jump, and properties of piecewise homogeneous Markov jump systems are discussed in~\cite{H_mj}. \fi

\iffalse There are several stable conceptions in literature, like the means square exponentially stable and mean square stable. \fi
\iffalse
\begin{definition}
The stochastic differential Equation is said to be exponentially stable in mean square if there is a pair of positive constants $\lambda$ and $M$ such that, for all initial data $x_0$, such that
\begin{align}
\mathbb{E}\|x_k\|^2 \leq M\mathbb{E}\|x_0\|^2 e^{-\lambda k}, \text{for all}\ k\geq 0.
\end{align}
\end{definition}

\begin{definition}
The stochastic differential equation is said to be mean square stable if 
\begin{align}
\lim\limits_{k\to\infty}\mathbb{E}\|x_k\|^2=0, \text{for any initial}\ \mathbf{x}_0, \sigma_0,
\end{align}
where $\sigma_0$ is the probability distribution of the initial subsystem. 
\end{definition}
\fi

%%%%%%%
%%%%%%%%%%
\iffalse
\begin{theorem}
When the Markov jump discrete time system is mean square stable, the nonstationary stochastic game has a stationary strategy as $k\to\infty$. 
\end{theorem}
\begin{proof}
\end{proof}
\fi
%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}
Consider the pure strategy of always applying the $j$-th controller (detector) at each stage for any attacker's strategy as a subsystem. Then the stochastic game strategy for the system is equivalent with randomly switching between $N$ controllers/detectors with any linear combination of probability $g_j, j \in \{1,\cdots, N\}, \sum_{j} g_j =1$, for any joint state. We assume every subsystem that equipped with a controller/detector can make the closed loop system mean square exponentially stable, even under worst case attack strategies (i.e., attacks can increase the system cost, but can not distablize the system), then for system always applying controller $j$, there exists a pair of positive constants $\lambda_j$ and $M_j$ such that, for all initial data $x_0$, such that
\begin{align}
\mathbb{E}\|x_k\|^2 \leq M_j\mathbb{E}\|x_0\|^2 e^{-\lambda_j k}, \text{for all}\ t\geq 0.
\end{align}
Then let $\lambda = min_{j \in N} \{\lambda_j\}, M= N max_{j\in N} \{M_j\}$, since $0\leq g_j \leq 1, 0\leq g_j^2\leq 1$,
\begin{align}
\begin{split}
\mathbb{E}\|\sum_j g_j x_k\|^2 &\leq \sum_j g_j^2 M_j\mathbb{E}\|x_0\|^2 e^{-\lambda_j k}\\
&\leq \sum_j M_j\mathbb{E}\|x_0\|^2 e^{-\lambda_j k}\\
&\leq M \mathbb{E}\|x_0\|^2 e^{-\lambda k},
\text{for all}\ k\geq 0.
\end{split}
\end{align}
The switching system according to the game strategy is also exponentially mean square stable.
\end{proof}
\fi


==> backup.tex <==
\section{Existence of An Optimal Strategy and Suboptimal Algorithm}
%\label{sec:algorithm_finite}

Based on the game formulation, in this section we discuss the existence of an optimal solution for the system, and present an algorithm to compute a suboptimal system strategy.%\PA{what do you mean by ``approximation computing algorithm''}
 
\subsection{Existence of the System's Optimal Strategy}

%Let the total number of game stages, $K$,  be a fixed positive integer, 
We define the concatenation of strategies for $K$-stage game of each player ($\mathbf{f}$ for attacker and $\mathbf{g}$ for system) as%\PA{notation is a bit confusing}
%\begin{align*}
%F^{K}:=\{\mathbf{f}=[\mathbf{f}^1,\cdots, \mathbf{f}^K]\},%\mathbf{f}^{k} \in \mathbf{F}_{k}\},\\ 
%G^{K}:=\{\mathbf{g}=[\mathbf{g}^{1},\cdots,\mathbf{g}^K]\}.%,\mathbf{g}^{k} %\in \mathbf{G}_{k}\}.
%\mathbf{F}=
\vspace{-4.5pt}
\begin{equation*}
\vspace{-4.5pt}
\mathbf{f}=\mathbf{f}_1\cdots \mathbf{f}_K,\mathbf{f}_{k} \in \mathbf{F}_{k},
%\mathbf{G}=
~~~~\mathbf{g}=\mathbf{g}_{1}\cdots\mathbf{g}_K,\mathbf{g}_{k} \in \mathbf{G}_{k}.
\end{equation*}
%\end{align*}
%Let $\zeta_{k}: H_{k} \to S$ denote the projections from $H^{k}$ onto the state space $S$ at stage $k$, then 
Let the random variable $\zeta_{k}$ describe the state of the game at stage $k$, and  
%The transition law $\mathbb{P}^{k}$, a strategy pair $f\in F^{K},g\in G^{K}$ define a conditional probability $P_{fg}(s^{1},.) : S\to A_{t1}\times A_{s1} \times \cdots A_{tK}\times A_{sK}$.$P_{fg} (s^{1},.)$ associates with each initial state $s^{1} \in S$ a probability measure on $H_{K}$, according to theorem of Ionescu-Tulcea ~\cite{Tulcea}. 
let us define the conditional expected total payoff till $\tilde{K}$ for any $\mathbf{f},\mathbf{g}$, given initial state $\zeta_{1}=s$ as%initial state $s$ as: 
\footnotesize
\begin{equation*}\vspace{-5pt}
R_{\tilde{K}}(s, \mathbf{f}, \mathbf{g})%=\sum \limits^{K}_{k=1} \mathbb{E}_{\mathbf{f}, \mathbf{g}}[\tilde{r}(h_k,\zeta_{k})|\zeta_{1} = s],\\
%& = -R_{K}^{s}(s,\mathbf{f}, \mathbf{g}) = R_{K}^{t}(s,\mathbf{f}, \mathbf{g})
%=\sum \limits^{K}_{k=1} \mathbb{E}_{\mathbf{f}, \mathbf{g}}[r(\zeta_{k},\mathbf{f},\mathbf{g})|\zeta_{1} = s],\\
%&\mathbb{E}_{\mathbf{f}, \mathbf{g}} [r(\zeta^{k},\mathbf{f},\mathbf{g})|\zeta^{1} = s]
=\sum \limits^{\tilde{K}}_{k=1}\sum_{l=1}^{3} p(\zeta_{k}=s_{l}|\zeta_{1} = s)[\mathbf{f}_{k}(s_{l})]^{T}\tilde{r}_{k}(h_{k},s_{l})\mathbf{g}_{k}(s_{l}).
\end{equation*}
\normalsize
%where For any given $\zeta_{1}=s$, strategy concatenation $\mathbf{f}, \mathbf{g}$, h_{k}=s\mathbf{f}^{1}\mathbf{g}^{1}\cdots\mathbf{f}^{k-1}\mathbf{g}^{k-1}$,
%\begin{align*}
%\mathbb{E} [r(\zeta_{k},\mathbf{f},\mathbf{g})]=\sum_{l=1}^{3} p(\zeta_{k}=s_{l})[\mathbf{f}^{k}(s_{l})]^{T}\tilde{r}^{k}(h^{k},s_{l})\mathbf{g}^{k}(s_{l}).
%\end{align*}
Since the immediate payoff satisfies $0 \leq \tilde{r}_{k}^{ij}(h_{k},s_{l})< \infty$, we have that $R_{\tilde{K}}(s, \mathbf{f}, \mathbf{g})$ is a nonnegative real-valued, nondecreasing function with $\tilde{K}$. 
%\PA{when you cut an old sentence to save space, make sure that the new one makes sense; for example you should have said - from the immediate payoff definition we have that ...' or ``since...''}  
Furthermore, for finite $K$%a finite stage game
%\PA{shouldn't it be ``for a finite game'' or ``for a finite stage game''}
\vspace{-4pt}
\begin{align}
%\sup_{\mathbf{f} \in F^{K}}R_{K}(s,\mathbf{f}, \mathbf{g}^{*}) < \infty,s \in S.
%\sup_{\mathbf{f}}
R_{K}(s,\mathbf{f}, \mathbf{g}) < \infty, \forall s, \mathbf{f}, \mathbf{g}.
\label{fR}
\end{align}
%%%%%%%%%%%
%%%%%%%%%%%%
\iffalse
Define the lower (upper) value function $\underbar{$v$}_{K,s}$ ($\bar{v}_{K,s}$) of the stochastic game as:
\begin{align*}
\underbar{$v$}_{K,s}=\sup_{\mathbf{f}\in F^{K}}\inf_{\mathbf{g}\in G^{K}}R_{K}(s,\mathbf{f}, \mathbf{g}),\\
\bar{v}_{K,s}=\inf_{\mathbf{g}\in G^{K}}\sup_{\mathbf{f}\in F^{K}}R_{K}(s,\mathbf{f}, \mathbf{g})
\end{align*}  
\fi
%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{definition}[\cite{finite_exist}]
A two-person zero-sum $K$-stage stochastic game 
%$\mathbf{\tilde{R}}(s) = [\tilde{r}(s, ]_{a_{j}\in A_{t}, u_{i} \in A_{s}}$ 
%at a particular state s 
is said to have a value vector $v^{*}_{K}$ if %or any $s\in S$,%\PA{not clear}
\begin{align*}
\begin{split}
&v^{*}_{K,s}=\underbar{$v$}_{K,s}=\bar{v}_{K,s},\ \text{for any}\ s\in S,\ \ \text{where}\\
&\underbar{$v$}_{K,s}= \sup_{\mathbf{f}}\inf_{\mathbf{g}}R_{K}(s,\mathbf{f}, \mathbf{g}),
~~~~\bar{v}_{K,s}=\inf_{\mathbf{g}}\sup_{\mathbf{f}}R_{K}(s,\mathbf{f},\mathbf{g}).
\end{split}
\end{align*}

%A strategy $\mathbf{f}^{*} \in F^{K}$ is called $\epsilon$-optimal for player one (the attacker) of the K-stage stochastic game if  for all $s\in S$
%\[\bar{v}_{K,s} \leq \inf_{\mathbf{g} \in G^{K}}R_{K}(s, \mathbf{f}^{*}, \mathbf{g}) + \epsilon,\]

For the finite value $K$-stage stochastic game, strategies $\mathbf{g}^{*}$ and $\mathbf{f}^{*}$ are called optimal for player two (the system) and player one (the attacker), respectively, if for all $s\in S$\\
%\vspace{-2pt}
%\begin{align*}
%\underbar{$v$}_{K,s} &\geq \sup_{\mathbf{f}}R_{K}(s, \mathbf{f}, \mathbf{g}^{*}) - \epsilon,\\
%\bar{v}_{K,s} &\leq \inf_{\mathbf{g}}R_{K}(s, \mathbf{f}^{*}, \mathbf{g}) + \epsilon.
$v^*_{K,s} = \sup\limits_{\mathbf{f}}R_{K}(s, \mathbf{f}, \mathbf{g}^{*}),%\\ - \epsilon,\\
~~v^*_{K,s} = \inf\limits_{\mathbf{g}}R_{K}(s, \mathbf{f}^{*}, \mathbf{g}). $%+ \epsilon.
%\end{align*}%The 0-optimal strategies are called optimal.
\end{definition}
%\begin{remark}
%The objective of security problems is usually ensuring the performance of the "weakest" link in the system. The value of the game defined in this paper is the minimum of the worst case cost for the system, which is consistent with security goal.
%\end{remark}

%\begin{lemma}%\cite{finite_exist}
The existence conditions of the value and optimal strategies for a general finite horizon zero-sum nonstationary stochastic game are shown in~\cite{finite_exist}. The game defined in this paper has a finite state space, finite action spaces, and satisfies~\eqref{fR}.
%the state transition probability and immediate payoff functions are defined to calculate the expectation total payoff, 
%and $\sup_{\mathbf{f} \in F^{K}}R_{K}(s,\mathbf{f}, \mathbf{g}^{*})$ is bounded.
%Our game model 
%\PA{adopted?} 
Therefore, using the same approach as in the proofs from~\cite{finite_exist} we can prove the following theorem:

\begin{theorem} 
%The value of the game and an optimal strategy for each player exist for the considered problem formulation.
There exists the value of the considered game and an optimal strategy for the system.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%
%%%%%%%%%%%%%%%
\iffalse
The game we define in this paper has properties: (i) for any stage k, the state space S, action space $A_{tk}$ for attacker and $A_{sk}$ for system are finite sets.   (ii) The state transition probability matrix $\tilde{P}^{k}(s_{h}|h_{k}, s_{l})$ together with the strategy history $h_{k}$ defines a conditional distribution for computing the expected total payoff. %at stage $k+1$, given the strategy history $h_{k} \in H_{k}$ and both players' actions at stage $k$. 
(iii) The immediate payoff $\tilde{r}^{k} (h_{k},s_{l})$ is nonnegative, and conditional expected total payoff function $R_{k}(s,\mathbf{f,g}): H_{K} \to R$ is a bounded below (nonnegative), nondecreasing, for $k\in\{1,\cdots,K\}$. %lower semicontinuous function on $H_{K}$. 
%(iv)In finite time, \[\sup_{\mathbf{f} \in F^{K}}R_{K}(s,\mathbf{f}, \mathbf{g}^{*}) < \infty,s \in S.\]
The game formulation in this paper can be interpreted by the abstract nonstationary game model in~\cite{finite_exist}, and a detail proof is provided in~\cite{finite_exist}.
%%%%\end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Suboptimal Algorithm For the Nonstationary Game}

Existing value iterative algorithms for stationary stochastic games can not be used to solve our game, since the nonstationary game parameters depend on the previous history, which is only available in the future algorithm iterations.
Hence, we design a suboptimal algorithm based on the  value iteration method for finite horizon stationary stochastic game from~\cite{plangame} and robust game techniques from~\cite{RGT}. 
Algorithm~\ref{finite} provides an upper bound for the game value and the corresponding nonstationary suboptimal strategy for the system. The idea is to solve a robust game at each iteration step -- i.e., minimize the worst-case caused by extreme points of the nonstationary payoff and state transition probability polyhedra, or $(r_{k},\mathbb{P}_{k})$, defined for all possible histories. 
%Algorithm~\ref{finite} for the finite horizon nonstationary stochastic game 

%The iteration works in the way, that if a player knew how to play in the robust stochastic game optimally from the next stage on, then, at the current stage, he would play with such strategies. Similar to a stationary stochastic game, this value iteration minimizes the maximum expected immediate cost at the current stage and expected costs possibly incurred in future stages.    
 
%
%The value iteration is: %such that for given initial $v^{0}_{s}$ the value of the game at time t+1 is:
%\begin{align*}
 %                     $v^{t}_{s}=\text{value}[\tilde{r}_{s}+\sum_{s'\in S} \tilde{P}(s'|s)v^{t+1}_{s'}].$
%\end{align*}
The value iteration algorithm for finite horizon stationary stochastic game (with fixed payoff $r$ and state transition probability $P$ at every stage) works in the way that if a player knew how to play in the game optimally from the next stage on, then, at the current stage, he would play with such strategies~\cite{plangame}. The value of $K$-stage game is finally provided by the last step of iteration. Similarly, the Algorithm~\ref{finite} of the nonstationary stochastic game starts from the last stage, gets the matrix game value and the optimal strategy related to nonstationary $(r_{k},\mathbb{P}_{k})$  at each stage, and returns an upper bound for the value of the total payoff in $K$-stages. 
To estimate the values %%%%iteration of 
at each step, we consider the payoff and state transition probability set ($r_{k}$, $\mathbb{P}_{k}$) as an uncertain parameter set for the one shot robust game~\cite{RGT}. %Then approximate each iteration value as the value of the robust one shot zero sum game. 

To quantify the bounded polyhedra ($r_{k}$, $\mathbb{P}_{k}$), we need the expected system dynamics $\mathbf{x}_{k}, \mathbf{u}_{k}$, $\mathbf{y}_{k}, k=1,\cdots,K$ defined in Section~\ref{dynamicgame}, which is determined by the strategy history.  
%(this approximation also holds for other attack game quantification model with bounded payoff and transition probability). 
The extreme points for the uncertain set  ($r_{k}$, $\mathbb{P}_{k}$) depend on pure strategy histories. Let $H^p_k \subset H_k$ be the concatenation of pure strategies until stage $k$, where  a pure history $h^{p}_{k} \in H^{p}_{k}$, $h^{p}_{k}=s_{1}\mathbf{f}^{p}_{1}\mathbf{g}^{p}_{1}\cdots\mathbf{f}^{p}_{k-1}\mathbf{g}^{p}_{k-1}$ satisfies that all $f^{p}_{t}(s), g^{p}_{t}(s)$ have only one non-zero element (i.e., they choose the corresponding action or the \emph{pure} strategy).  
By using any $h^{p}_{k}$ in the game model of Section~\ref{dynamicgame}, we get the corresponding $r^p_k(h^p_k,s_l)$ and $P^p_k(h^p_k,s_l)$ for stages $1$ to $K$. Thus, the extreme points set $(r_{kp},\mathbb{P}_{kp})$ for $(r_{k}, \mathbb{P}_{k})$ is:%which we define as: \\
%\vspace{-4pt}
\begin{equation*}
\{(r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(h^{p}_{k},s_{l})) |~h^{p}_{k}\in H^{p}_{k},l\in\{1,2,3\}\}.
\end{equation*}
%\vspace{-4pt}
%%%%%%%%%%%%%%%


\iffalse
Now, consider the iteration for calculating the pure history value $v_{k}^{s_{l}}(h^{p}_{k})$ (from extreme points $(r_{kp},\mathbb{P}_{kp})$). %based on $v_{k+1}^{s'}(h^{p}_{k+1})$ of the previous inductive value iteration process at $k+1$.
We denote the non-pure history value of $k$ as $v_{k}^{s_{l}}(h^{p}_{k-1})$, which is calculated from the $(r_k,\mathbb{P}_k)$ that have pure strategies in all stages $1,\cdots,k-2$, and any strategy at stage $k-1$.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%



We define the pure strategy backup matrix set $\mathbb{Q}_{kp}$, $k=1,\cdots,K-1$ as:
%for each $(r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(h^{p}_{k},s_{l}))\in (r_{kp},\mathbb{P}_{kp})$,
\vspace{-5pt}
\footnotesize
\begin{align}
\vspace{-5pt}
\mathbb{Q}_{kp}=\{Q_{k}^{p}(h^{p}_{k},s_{l}) = r^{p}_{k}(h^{p}_{k},s_{l})+\sum_{s'\in S} P^{p}_{k}( s' |h^{p}_{k},s_{l})v_{k+1}^{s'}(h^{p}_{k+1})\},
\label{eq:Q}
\end{align}
\normalsize
where $v^{s'}_{k+1}(h^p_{k+1})\geq 0$ is the robust game value resulting from the iteration at stage $k+1$ of~Algorithm~\ref{finite}, and relates to matrix games defined by $\mathbb{Q}_{(k+1)p}$.
 In addition,  we define the backup matrix set~$\mathbb{Q}_{k}$ for all possible~$h_{k}$,  as
 
\vspace{-8pt}
\footnotesize
\begin{align*}
\vspace{-5pt}
\mathbb{Q}_{k}= 
\{&\tilde{Q}_{k}(h_{k},s_{l})=\tilde{r}_{k}(h_{k},s_{l})+\sum_{s'\in S}\tilde{P}_{k}(s'|h_{k},s_{l})v^{s'}_{k+1}(h^p_{k+1})\}.
%&h_{k} \in H_{k}, l=1,2,3\}.
\end{align*} 
\normalsize
Finally, for the stage $K$ we define $Q_{K}^{p}(h^{p}_{K},s_{l})= r^{p}_{K}(h^{p}_{K},s_{l})$ and $\tilde{Q}_{K}(h_{K},s_{l})=\tilde{r}_{K}(h_{K},s_{l})$. 

Now, consider the iteration for calculating $v_{k}^{s_{l}}(h^{p}_{k})$ from all matrix games $Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}$ in Algorithm~\ref{finite}. 
We denote the non-pure history value of $k$ as $v_{k}^{s_{l}}(h^{p}_{k-1})$, which is calculated from the $\tilde{Q}_{k}(h_{k},s_{l})$ that have the same pure strategies as $h^p_k$ in all stages $1,\cdots,k-2$, and any strategy at stage $k-1$.
We use the following result to show that  at every $k$, $v_{k}^{s_{l}}(h^{p}_{k})$ is greater than or equal to $v_{k}^{s_{l}}(h^{p}_{k-1})$.


\begin{theorem}
Consider the value iteration for stage $k$ as a one shot robust game. %given a pure strategy history $h^{p}_{k}$, 
Based on $v_{k+1}^{s'}(h^{p}_{k+1}) \geq 0$ of previous iteration, 
We define the robust game value  obtained at $k$ as %to compute $v^{k-1}_{s}(h^{p}_{k-1})$ at $k-1$ as:
\begin{align}
v^{s_{l}}_{k}(h_{k}^{p})=\max_{Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}}v^*[Q_{k}^{p}(h^{p}_{k},s_{l})],%v_{k}^{s_{l}}(h_{k}^{p})&=\max_{(r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(h^{p}_{k},s_{l}))}
%v^*[r^{p}_{k}(h^{k}_{p},s_{l})+\sum_{s'\in S} P^{p}_{k}( s' |h^{p}_{k},s_{l})v_{k+1}^{s'}(h^{p}_{k+1})],
\label{pickv}
\end{align}
where $v^*$ is the function that yields the value of a zero-sum matrix game. Then for $k=2,\cdots, K$, $v_{k}^{s_{l}}(h^{p}_{k-1})$ is upper bounded by $v_{k}^{s_{l}}(h_{k}^{p})$ (i.e.,~$v^{s_{l}}_{k}(h^{p}_{k-1})\leq v_{k}^{s_{l}}(h_{k}^{p})$).%&\max_{(r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(\cdot|h^{p}_{k},s_{l}))\in (r^{kp},\mathbb{P}^{kp})}%\in (M^{p}_{ks_{l}}(h^{p}_{k}), P^{p}_{k}( . |h^{p}_{k},s_{l}))}\\
%\text{value}[r^{p}_{k}(h^{k}_{p},s_{l})+\\
%&\sum_{s'\in S} P^{p}_{k}( s' |h^{p}_{k},s_{l})v^{k+1}_{s'}(h^{p}_{k})].
%\end{align*}
 %and we have exact 4 $v^{k+1}_{s'}(h^{p}_{k})$ for every $s' \in S$ as candidate backup value at every stage k. 
\label{robust}
\end{theorem}


\begin{proof}
%In the following proof every $h_{k}^{p}$ is a branch for the same $h^{p}_{k-1}$, $h_{k}=h_{k-1}^{p}\mathbf{f}^{k}\mathbf{g}^{k}$, and we omit the subscript $h^{p}_{k-1}$. 
\iffalse
The backup matrix set $\mathbb{Q}_{k}$ for all possible $h_{k}$ is %for $s_l$ :
\begin{align*}
%Q_{k}= 
\{&\tilde{Q}_{k}(h_{k},s_{l})=\tilde{r}_{k}(h_{k},s_{l})+\sum_{s'\in S}\tilde{P}_{k}(s'|h_{k},s_{l})v^{s'}_{k+1}(h_{k+1}^{p})\},
%&h_{k} \in H_{k}, l=1,2,3\}.
\end{align*}
\fi
%%%%%%%%%%%%%%%%%%%%%
%$\tilde{Q}_{k}\in \mathbb{Q}_k$. 
Since $v^{s'}_{k+1}(h_{k+1}^{p})$ is a nonnegative scalar, the extreme points of $\mathbb{Q}_{k}$ can only come from the extreme points of the tuple $(r_{k}, \mathbb{P}_{k})$, i.e., by considering the matrix game value of every $Q_{k}^{p} (h_{k}^{p},s_{l})$ defined in~\eqref{eq:Q}, we will get the maximum value from extreme points of $\mathbb{Q}_k$. 
%\[\tilde{Q}_{k}^{p}=\{ Q_{k}^{p} (h_{k}^{p},s_{l}), (r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(h^{p}_{k},s_{l}))\in (r^{kp},\mathbb{P}^{kp})\}.\] 
%we only need to consider every extreme point  $(r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(\cdot|h^{p}_{k},s_{l}))$ in
% 
Now consider the following optimization problem for the system~\eqref{optr} and for any attacker's strategy vector $\mathbf{f}$
%From the system's perspective, to compute the value of the matrix game is equivalent with:
\vspace{-5pt}
\begin{align}
%\begin{split}
\vspace{-5pt}
\min_{\mathbf{g}} \quad & z\label{ob_z}\\
\text{subject to}\quad &z \geq \max_{\tilde{Q}_{k}(h_{k},s_{l})\in \mathbb{Q}_{k}}\mathbf{f}^{T} [\tilde{Q}_{k}(h_{k},s_{l})]\mathbf{g}.
%\end{split}
\label{optr}
\end{align}
As proven by~Lemma 5 in \cite{RGT},~\eqref{optr} is equivalent to the following constraint that considers only the extreme points
\begin{align}
\quad z \geq \max_{Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}}\mathbf{f}^{T} [Q_{k}^{p}(h^{p}_{k},s_{l})]\mathbf{g},
\end{align}
%meaning that it is sufficient to consider only the extreme points.


For the worst-case $f$, the above is also true. Hence, let 
\begin{align}
\label{eq1}
v^{s_{l}}_{k}(h_{k}^{p})
%=\max_{Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}}v^*[Q_{k}^{p}(h^{p}_{k},s_{l})]
=\max_{Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}} \min\limits_{\mathbf{g}}\max\limits_{\mathbf{f}}\mathbf{f}^T[Q_{k}^{p}(h^{p}_{k},s_{l})]\mathbf{g}.
%\label{pickv}
\end{align}
For optimal policies $\mathbf{f}^{*}(h^{p}_{k},s_{l})$ and $\mathbf{g}^{*} (h^{p}_{k},s_{l})$, the above optimization \eqref{eq1} results in cost $\max\limits_{Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}}v^*[Q_{k}^{p}(h^{p}_{k},s_{l})]$. 
%we can compute the value from four different $\tilde{Q}_{ks_{l}}^{p}(h^{p}_{k})$separately, and get the value follow the pure strategy $v^{k}_{s'}(h^{p}_{k-1})$. 
However, $(\mathbf{f}^{*}(h^{p}_{k},s_{l}),\mathbf{g}^{*}(h^{p}_{k},s_{l}))$ can be non-pure strategies, meaning that when used in~\ref{dynamicgame}, they will not result in extreme points of $\mathbb{Q}_{k+1}$. The non-pure history value $v_{k+1}^{s'}(h_{k}^{p})$ of iteration for stage $k+1$ satisfies %%%%%(from $\mathbb{Q}_{(k+1)p}$):
%\begin{align*}
$
v_{k+1}^{s'}(h_{k}^{p})\leq v_{k+1}^{s'}(h_{k+1}^{p}). 
$
%\end{align*}
Replacing $v_{k+1}^{s'}(h_{k+1}^{p})$ by $v_{k+1}^{s'}(h_{k}^{p})$ in~\eqref{eq:Q} will decrease every element in matrix $Q^{p}_{k}$, since $r_{k}^{ij}\geq0$ and $P_{k}^{ij}\geq 0$. %%% by definition. 
%The system is a minimizer, and is possible to get a smaller value at time k, with some %optimal strategy history $h^{*}_{k} \neq h^{p}_{k}$, 
With a similar argument in the next iteration for stage $k-1$, we have $v_{k}^{s_{l}}(h^{p}_{k-1})\leq v^{s_{l}}_{k}(h_{k}^{p})$. 
%(Note that here $v_{k}^{s_{l}}(h^{p}_{k-1})$ is not the game value at $k$ either, because the strategies from 1 to $k-2$ must be pure to get it).
\end{proof}
%\squeezeup
%\vspace{-5pt}
\begin{algorithm}
%\vspace{-5pt}
\caption{\textbf{: Suboptimal Algorithm for A Finite Nonstationary  Stochastic Game }}
\textbf{Input}: System model parameters and game parameters.
\\\textbf{Initialization}:
             Compute the set of $(r_{kp}, \mathbb{P}_{kp})$ for $k=1,...K$.
              %For all $s_{l} \in S, l =1,2,3, h^{p}_{K}\in H^{p}_{K} :$ get %$4^{K-1}$ 
              %backup matrix set $\{Q_{k}^{p}(h_{k}^{p},s_{l})\}$:
              
             Compute the game at stage $K$: $Q_{K}^{p}(h^{p}_{K},s_{l})=r_{K}^{p}(h^{p}_{K},s_{l})$, \\ 
                    $f^{*}(h^{p}_{K}, s_{l}), g^{*}(h^{p}_{K}, s_{l}), v_{K}^{s_{l}}(h^{p}_{K}) \leftarrow \pi(Q_{K}^{p}(h^{p}_{K},s_{l}).$
\\\textbf{Iteration}: For $k=(K-1), \cdots, 1$,

get the backup matrix set $\mathbb{Q}_{kp}$ for all $h^{p}_{k}\in H^{p}_{k}$, where each matrix is defined in~\eqref{eq:Q}, then calculate:
%\[Q_{k}^{p}(h^{p}_{k},s_{l}) = r^{p}_{k}(h^{p}_{k},s_{l})+\sum_{s'\in S} P^{p}_{k}( s' |h^{p}_{k},s_{l})v_{k+1}^{s'}(h^{p}_{k+1}),\]

 $f^{*}(h^{p}_{k}, s_{l}), g^{*}(h^{p}_{k}, s_{l}),v_{k}^{s_{l}}(h^{p}_{k}) \leftarrow \pi(Q_{k}^{p}(h^{p}_{k},s_{l}))$.
 
%$\mathbf{f}^*_k=[\mathbf{f}^{*}(h^{p}_{k}, s_{l}),\mathbf{f}^{*}(h^{p}_{k}, s_{2}), \mathbf{f}^{*}(h^{p}_{k}, s_{3})],$ $ \mathbf{g}^{*}_k=[\mathbf{g}(h^{p}_{k}, s_{1}),\mathbf{g}(h^{p}_{k}, s_{2}),\mathbf{g}(h^{p}_{k}, s_{3})].$ 

$\mathbf{f}^*_k=[\mathbf{f}^{*}(h^{p}_{k}, s_{l}),l=1,2,3],$ $ \mathbf{g}^{*}_k=[\mathbf{g}^*(h^{p}_{k}, s_{l}), l=1,2,3].$ 

\textbf{Return}: the strategy concatenation pair $\mathbf{f}_{a}=\mathbf{f}^{*}_1\cdots\mathbf{f}^*_K,\mathbf{g}_{a}=\mathbf{g}^{*}_1\cdots\mathbf{g}^*_K$ and the value upper bound $v^{s_{l}}_{1},l=1,2,3$.
\label{finite}
%\vspace{-5pt}
\end{algorithm}
%\squeezeup

According to~Theorem~\ref{robust}, we use Algorithm~\ref{finite} to compute an upper bound of the value and the corresponding suboptimal strategy for every step. The % Nash Equilibrium selection 
function $\pi$ computes the strategy and robust value as defined in~\eqref{pickv}. Note that for the replay attacks considered in this paper, at state $s_{1}$ the system wins the game and replay is harmless. Thus, the optimal strategies of $s_{1}$ is $\mathbf{g}_{k}(s_{1})=\begin{bmatrix}1&0\end{bmatrix}^{T}$, $\mathbf{f}_{k}(s_{1})=\begin{bmatrix}1&0&\cdots&0\end{bmatrix}^{T}$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%the Input can be: $\mathbf{A,B,C,Q,R,\bar{x}_{0}},\Sigma,$ $\mathbf{K},$ $\mathbf{W,U,L}$, $\tau, \alpha, \Delta \mathbf{u}_{k}\sim N(0,\mathcal{L})$; replay window size $\{t_{2},\cdots,t_{M}\}$, total stage number $K$, system initial state distribution $p(s^{1})$, false alarm trigger penalty.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The nonstationary game values $v_k^{s_l}(h^p_{k-1})$ and $v_k^{s_l}(h^p_k)$ that result from value iteration of two strategies only differ at stage $k-1$ (i.e.,~same and pure from stages 1 to $k-2$). By value iteration backward to stage 1, we compare the game value (for all possible strategies) and the robust game value $v_1^{s_l}$ of~Algorithm~\ref{finite} in the following theorem.
\begin{theorem}
%Moreover, by following this iteration method,
~Algorithm~\ref{finite} results  in an upper bound $v_{1}^{s_{l}}$ for the value of the $K$-stage game, together with suboptimal strategies $\mathbf{f}_{a}$ and $\mathbf{g}_{a}$. 
\end{theorem}
\vspace{3pt}
\begin{proof}
The strategies $\mathbf{f}_{a}, \mathbf{g}_{a}$ of~Algorithm~\ref{finite} are possibly not pure. %strategy history $h^{p}_{K} \in H^{p}_{K}$. 
According to~Theorem~\ref{robust}, $v_{k}^{s_{l}}(h^{p}_{k-1})\leq v^{s_{l}}_{k}(h_{k}^{p})$, %(may write this proof more detailed depends on the paper requirement)
and the proof holds for every $k=2,\cdots,K$.  \iffalse Using induction,\fi Consider the value iteration for $k=1$, with $v_{2}^{s_{l}}(h^{p}_{1})\leq v^{s_{l}}_{2}(h_{2}^{p})$, 
\footnotesize
\begin{equation*}
\vspace{-5pt}
Q_1^{ij}(h_1, s_l)=\tilde{r}_1^{ij}(h_1,s_l)+\sum\limits_{s'\in S}\tilde{P}^{ij}_{1}(s'|h_{1},s_{l})v^{s'}_{2}(h^p_{1})\leq Q_1^{ij}(h_2^p,s_l),
\end{equation*}
\normalsize
thus $v^{*}[Q_1(h_1, s_l)] \leq v^{s_{l}}_{1}$.  Iterative value based on pure strategy back up matrix sets $\mathbb{Q}_{kp}, k=1,\cdots, K$ obtained from~Algorithm~\ref{finite} is an upper bound for the game value.
\end{proof}

\iffalse
\begin{remark} %%%%%\FM{remove this remark to the extension paper?}
Algorithm~\ref{finite} is exponential with K, and for large control system running time $\tilde{T}$, the game stage $K$ does not need to be $\tilde{T}$--% We can formulate a $K$-stage game, 
each stage we compute $\tilde{T}/K$ steps of control system dynamic, and apply the average cost and transition probability to quantify the game parameters. 
%keeps the same during each stage ($\tilde{T}/K$ time).  
In particular, if we consider the infinite horizon problem, the game formulation can reduce to stationary. 
For example, we can define the infinite time average LQG cost as the payoff function, and the average detection rate/false alarm trigger rate as state transition probability, and find the optimal strategy of a stationary stochastic game.
%Or assume the replay window size does not change during K.
\end{remark}%\FM{we can put this remark at the end of section 3?}
\fi

\iffalse
Besides finding the optimal or suboptimal strategy, we can also use the stochastic game framework to find the `best reply' strategy for a specific attacker behavior. For example, the attacker's strategy can be to always apply a certain type of attack before being detected. When we want a faster iteration, we can calculate the best reply strategy with respect to one attack type from the attacker's action space, run the algorithm for a different action type each time, 
and find the worst-case cost. This approximation is reasonable, since when we do not have expectation that a certain attack type will appear, then our goal is to keep the system performance acceptable under the worst-case attack events.\fi

  %$(4\times2)$ action space (i.e., the attacker has 4 actions and the system has 2 actions).
  %This is because the computation complexity of the real-time algorithm grows linearly with the total stage number $K$, whereas the suboptimal algorithm is exponential with respect to $K$. 
  %As shown in Table~\ref{alg_compare}, the computation overhead of the suboptimal algorithm in~\cite{cdc_replay} increases faster with the total stage $K$ than that of Algorithm~\ref{finite_new}.

\iffalse
To get a suboptimal total payoff of time $\tilde{T}$ faster, we can view this as a $K$ stage game, and at each stage the physical dynamics run $[\tilde{T}/K]$ steps as~\eqref{eq:xu}. The average payoff and state transition probability in the $[\tilde{T}/K]$ discrete time slots are the payoff and state transition probability of one game stage.  
In particular, when we consider the average of infinite horizon time $\tilde{T}$, the game can reduce to a stationary stochastic game. For example, with the infinite time average LQG cost as the payoff function, and the average detection rate, false alarm trigger rate as the state transition probability, we actually reach the optimal strategy of a stationary stochastic game.  
\fi

%For the discrete time switched system switches among stable and unstable subsystems, where the transition probability is determined by the game strategy, the stability property still needs future analysis.
\iffalse the system is still Markov jump, and properties of piecewise homogeneous Markov jump systems are discussed in~\cite{H_mj}. \fi

\iffalse There are several stable conceptions in literature, like the means square exponentially stable and mean square stable. \fi
\iffalse
\begin{definition}
The stochastic differential Equation is said to be exponentially stable in mean square if there is a pair of positive constants $\lambda$ and $M$ such that, for all initial data $x_0$, such that
\begin{align}
\mathbb{E}\|x_k\|^2 \leq M\mathbb{E}\|x_0\|^2 e^{-\lambda k}, \text{for all}\ k\geq 0.
\end{align}
\end{definition}

\begin{definition}
The stochastic differential equation is said to be mean square stable if 
\begin{align}
\lim\limits_{k\to\infty}\mathbb{E}\|x_k\|^2=0, \text{for any initial}\ \mathbf{x}_0, \sigma_0,
\end{align}
where $\sigma_0$ is the probability distribution of the initial subsystem. 
\end{definition}
\fi

%%%%%%%
%%%%%%%%%%
\iffalse
\begin{theorem}
When the Markov jump discrete time system is mean square stable, the nonstationary stochastic game has a stationary strategy as $k\to\infty$. 
\end{theorem}
\begin{proof}
\end{proof}
\fi
%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{proof}
Consider the pure strategy of always applying the $j$-th controller (detector) at each stage for any attacker's strategy as a subsystem. Then the stochastic game strategy for the system is equivalent with randomly switching between $N$ controllers/detectors with any linear combination of probability $g_j, j \in \{1,\cdots, N\}, \sum_{j} g_j =1$, for any joint state. We assume every subsystem that equipped with a controller/detector can make the closed loop system mean square exponentially stable, even under worst case attack strategies (i.e., attacks can increase the system cost, but can not distablize the system), then for system always applying controller $j$, there exists a pair of positive constants $\lambda_j$ and $M_j$ such that, for all initial data $x_0$, such that
\begin{align}
\mathbb{E}\|x_k\|^2 \leq M_j\mathbb{E}\|x_0\|^2 e^{-\lambda_j k}, \text{for all}\ t\geq 0.
\end{align}
Then let $\lambda = min_{j \in N} \{\lambda_j\}, M= N max_{j\in N} \{M_j\}$, since $0\leq g_j \leq 1, 0\leq g_j^2\leq 1$,
\begin{align}
\begin{split}
\mathbb{E}\|\sum_j g_j x_k\|^2 &\leq \sum_j g_j^2 M_j\mathbb{E}\|x_0\|^2 e^{-\lambda_j k}\\
&\leq \sum_j M_j\mathbb{E}\|x_0\|^2 e^{-\lambda_j k}\\
&\leq M \mathbb{E}\|x_0\|^2 e^{-\lambda k},
\text{for all}\ k\geq 0.
\end{split}
\end{align}
The switching system according to the game strategy is also exponentially mean square stable.
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{proposition}
If the control input $\gamma(a_{ik}, u_{jk})=L_j\hat{\mathbf{x}}_{t}, t\in[k-T, k]$ for any action pair $(a_{ik}, u_{jk})$, then the system is not asymptotically stable when the strategy sequences $\mathbf{f}_k^*(s_{kl})$, $\mathbf{g}_k^*(s_{kl})$ of the stochastic game are not convergent.
\end{proposition}
%\begin{proof}

Sketch of the proof: 
When the system is asymptotically stable, $\lim_{k\to\infty}\mathbf{Ex}_k=0$, by the definition of immediate payoff function~\eqref{payoff}, we gave $$
After calculating the strategies at stage $k$, the next step of the Algorithm~\ref{finite_new} is updating the system dynamics, and then getting the auxiliary matrices $Q_{k}(s_{(k+1)l}),l=1,2,3$ for stage $k+1$. 
%\end{proof}
\fi

\iffalse After calculating the strategies at stage $k$, the next step of the Algorithm~\ref{finite_new} is updating the system dynamics, and then getting the auxiliary matrices $Q_{k}(s_{(k+1)l}),l=1,2,3$ for stage $k+1$. 
The saddle-point equilibrium strategies at stage $k+1$ are decided by $Q_{k}(s_{(k+1)l}),l=1,2,3$. 
Thus, if updating the system dynamics for the auxiliary matrix $Q_{k}(s_{kl})$ and at each mode $Q_{k}(s_{kl})$  converges with an optimal strategy for both players, \fi


\iffalse
If $(A+BL)(I-KC) \triangleq \mathcal{A}$ is stable, the $\chi^2$ detector is useless, since 
the expectation of detector statistics for the compromised residues $\mathbf{z}'_k=\mathbf{y}_{k-T}-\mathbf{C\hat{x}}_{k|k-1}$ will converge to the same value as that for $\mathbf{z}_k=\mathbf{y}_{k} -\mathbf{C\hat{x}}_{k|k-1}$~\cite{replay}
\begin{align}
\begin{split}
&\lim \limits_{k \to \infty} \mathbb{E}[(\mathbf{z}'_k)^{T} \mathcal{P}^{-1}\mathbf{z}'_k]=\lim \limits_{k \to \infty} \mathbb{E}[(\mathbf{z}_k)^{T} \mathcal{P}^{-1}\mathbf{z}_k]=m
%&\lim \limits_{k \to \infty} \mathbb{E}[(\mathbf{y}_{k} -\mathbf{C\hat{x}}_{k|k-1})^{T} \mathcal{P}^{-1} (\mathbf{y}_{k} - \mathbf{C\hat{x}}_{k|k-1})]=m
%&\lim \limits_{k \to \infty} E[(\mathbf{y}_{k-T} - \mathbf{C\hat{x}}_{k|k-1})^{T} \mathcal{P}^{-1} (\mathbf{y}_{k-T} - \mathbf{C\hat{x}}_{k|k-1})]=m,
\end{split}
\label{Er}
\end{align}
\normalsize
\fi

\iffalse the Kalman filter residue $\mathbf{z}'_k$ satisfy:
\begin{align*}
\begin{split}
&\lim \limits_{k \to \infty} \mathbb{E}[(\mathbf{z}'_k)^{T} \mathcal{P}^{-1}\mathbf{z}'_k]=m + 2 trace(\mathbf{C}^{T}\mathcal{P}^{-1}\mathbf{C}\mathcal{U}), \ \ \text{while}\\
&\lim \limits_{k \to \infty} \mathbb{E}[(\mathbf{z}_k)^{T} \mathcal{P}^{-1}\mathbf{z}_k]=m,
\mathcal{U} - \mathbf{B}\mathcal{L} \mathbf{B}^{T} = \mathcal{AUA}^{T}.
\end{split}
\end{align*}
\fi


\iffalse
The game we define in this paper has properties: (i) for any stage k, the state space S, action space $A_{tk}$ for attacker and $A_{sk}$ for system are finite sets.   (ii) The state transition probability matrix $\tilde{P}^{k}(s_{h}|h_{k}, s_{l})$ together with the strategy history $h_{k}$ defines a conditional distribution for computing the expected total payoff. %at stage $k+1$, given the strategy history $h_{k} \in H_{k}$ and both players' actions at stage $k$. 
(iii) The immediate payoff $\tilde{r}^{k} (h_{k},s_{l})$ is nonnegative, and conditional expected total payoff function $R_{k}(s,\mathbf{f,g}): H_{K} \to R$ is a bounded below (nonnegative), nondecreasing, for $k\in\{1,\cdots,K\}$. %lower semicontinuous function on $H_{K}$. 
%(iv)In finite time, \[\sup_{\mathbf{f} \in F^{K}}R_{K}(s,\mathbf{f}, \mathbf{g}^{*}) < \infty,s \in S.\]
The game formulation in this paper can be interpreted by the abstract nonstationary game model in~\cite{finite_exist}, and a detail proof is provided in~\cite{finite_exist}.
%%%%\end{proof}
\fi

==> ne_exist.tex <==
\section{Existence of An Optimal Strategy and Suboptimal Algorithm}
\label{sec:ne1}

Based on the game formulation, in this section we discuss the existence of an optimal solution for the system, and present an algorithm to compute a suboptimal system strategy.%\PA{what do you mean by ``approximation computing algorithm''}
 
\subsection{Existence of the System's Optimal Strategy}

%Let the total number of game stages, $K$,  be a fixed positive integer, 
We define the concatenation of strategies for $K$-stage game of each player ($\mathbf{f}$ for attacker and $\mathbf{g}$ for system) as%\PA{notation is a bit confusing}
%\begin{align*}
%F^{K}:=\{\mathbf{f}=[\mathbf{f}^1,\cdots, \mathbf{f}^K]\},%\mathbf{f}^{k} \in \mathbf{F}_{k}\},\\ 
%G^{K}:=\{\mathbf{g}=[\mathbf{g}^{1},\cdots,\mathbf{g}^K]\}.%,\mathbf{g}^{k} %\in \mathbf{G}_{k}\}.
%\mathbf{F}=
\vspace{-4.5pt}
\begin{equation*}
\vspace{-4.5pt}
\mathbf{f}=\mathbf{f}_1\cdots \mathbf{f}_K,\mathbf{f}_{k} \in \mathbf{F}_{k},
%\mathbf{G}=
~~~~\mathbf{g}=\mathbf{g}_{1}\cdots\mathbf{g}_K,\mathbf{g}_{k} \in \mathbf{G}_{k}.
\end{equation*}
%\end{align*}
%Let $\zeta_{k}: H_{k} \to S$ denote the projections from $H^{k}$ onto the state space $S$ at stage $k$, then 
Let the random variable $\zeta_{k}$ describe the state of the game at stage $k$, and  
%The transition law $\mathbb{P}^{k}$, a strategy pair $f\in F^{K},g\in G^{K}$ define a conditional probability $P_{fg}(s^{1},.) : S\to A_{t1}\times A_{s1} \times \cdots A_{tK}\times A_{sK}$.$P_{fg} (s^{1},.)$ associates with each initial state $s^{1} \in S$ a probability measure on $H_{K}$, according to theorem of Ionescu-Tulcea ~\cite{Tulcea}. 
let us define the conditional expected total payoff till $\tilde{K}$ for any $\mathbf{f},\mathbf{g}$, given initial state $\zeta_{1}=s$ as%initial state $s$ as: 
\footnotesize
\begin{equation*}\vspace{-5pt}
R_{\tilde{K}}(s, \mathbf{f}, \mathbf{g})%=\sum \limits^{K}_{k=1} \mathbb{E}_{\mathbf{f}, \mathbf{g}}[\tilde{r}(h_k,\zeta_{k})|\zeta_{1} = s],\\
%& = -R_{K}^{s}(s,\mathbf{f}, \mathbf{g}) = R_{K}^{t}(s,\mathbf{f}, \mathbf{g})
%=\sum \limits^{K}_{k=1} \mathbb{E}_{\mathbf{f}, \mathbf{g}}[r(\zeta_{k},\mathbf{f},\mathbf{g})|\zeta_{1} = s],\\
%&\mathbb{E}_{\mathbf{f}, \mathbf{g}} [r(\zeta^{k},\mathbf{f},\mathbf{g})|\zeta^{1} = s]
=\sum \limits^{\tilde{K}}_{k=1}\sum_{l=1}^{3} p(\zeta_{k}=s_{l}|\zeta_{1} = s)[\mathbf{f}_{k}(s_{l})]^{T}\tilde{r}_{k}(h_{k},s_{l})\mathbf{g}_{k}(s_{l}).
\end{equation*}
\normalsize
%where For any given $\zeta_{1}=s$, strategy concatenation $\mathbf{f}, \mathbf{g}$, h_{k}=s\mathbf{f}^{1}\mathbf{g}^{1}\cdots\mathbf{f}^{k-1}\mathbf{g}^{k-1}$,
%\begin{align*}
%\mathbb{E} [r(\zeta_{k},\mathbf{f},\mathbf{g})]=\sum_{l=1}^{3} p(\zeta_{k}=s_{l})[\mathbf{f}^{k}(s_{l})]^{T}\tilde{r}^{k}(h^{k},s_{l})\mathbf{g}^{k}(s_{l}).
%\end{align*}
Since the immediate payoff satisfies $0 \leq \tilde{r}_{k}^{ij}(h_{k},s_{l})< \infty$, we have that $R_{\tilde{K}}(s, \mathbf{f}, \mathbf{g})$ is a nonnegative real-valued, nondecreasing function with $\tilde{K}$. 
%\PA{when you cut an old sentence to save space, make sure that the new one makes sense; for example you should have said - from the immediate payoff definition we have that ...' or ``since...''}  
Furthermore, for finite $K$%a finite stage game
%\PA{shouldn't it be ``for a finite game'' or ``for a finite stage game''}
\vspace{-4pt}
\begin{align}
%\sup_{\mathbf{f} \in F^{K}}R_{K}(s,\mathbf{f}, \mathbf{g}^{*}) < \infty,s \in S.
%\sup_{\mathbf{f}}
R_{K}(s,\mathbf{f}, \mathbf{g}) < \infty, \forall s, \mathbf{f}, \mathbf{g}.
\label{fR}
\end{align}
%%%%%%%%%%%
%%%%%%%%%%%%
\iffalse
Define the lower (upper) value function $\underbar{$v$}_{K,s}$ ($\bar{v}_{K,s}$) of the stochastic game as:
\begin{align*}
\underbar{$v$}_{K,s}=\sup_{\mathbf{f}\in F^{K}}\inf_{\mathbf{g}\in G^{K}}R_{K}(s,\mathbf{f}, \mathbf{g}),\\
\bar{v}_{K,s}=\inf_{\mathbf{g}\in G^{K}}\sup_{\mathbf{f}\in F^{K}}R_{K}(s,\mathbf{f}, \mathbf{g})
\end{align*}  
\fi
%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{definition}[\cite{finite_exist}]
A two-person zero-sum $K$-stage stochastic game 
%$\mathbf{\tilde{R}}(s) = [\tilde{r}(s, ]_{a_{j}\in A_{t}, u_{i} \in A_{s}}$ 
%at a particular state s 
is said to have a value vector $v^{*}_{K}$ if %or any $s\in S$,%\PA{not clear}
\begin{align*}
\begin{split}
&v^{*}_{K,s}=\underbar{$v$}_{K,s}=\bar{v}_{K,s},\ \text{for any}\ s\in S,\ \ \text{where}\\
&\underbar{$v$}_{K,s}= \sup_{\mathbf{f}}\inf_{\mathbf{g}}R_{K}(s,\mathbf{f}, \mathbf{g}),
~~~~\bar{v}_{K,s}=\inf_{\mathbf{g}}\sup_{\mathbf{f}}R_{K}(s,\mathbf{f},\mathbf{g}).
\end{split}
\end{align*}

%A strategy $\mathbf{f}^{*} \in F^{K}$ is called $\epsilon$-optimal for player one (the attacker) of the K-stage stochastic game if  for all $s\in S$
%\[\bar{v}_{K,s} \leq \inf_{\mathbf{g} \in G^{K}}R_{K}(s, \mathbf{f}^{*}, \mathbf{g}) + \epsilon,\]

For the finite value $K$-stage stochastic game, strategies $\mathbf{g}^{*}$ and $\mathbf{f}^{*}$ are called optimal for player two (the system) and player one (the attacker), respectively, if for all $s\in S$\\
%\vspace{-2pt}
%\begin{align*}
%\underbar{$v$}_{K,s} &\geq \sup_{\mathbf{f}}R_{K}(s, \mathbf{f}, \mathbf{g}^{*}) - \epsilon,\\
%\bar{v}_{K,s} &\leq \inf_{\mathbf{g}}R_{K}(s, \mathbf{f}^{*}, \mathbf{g}) + \epsilon.
$v^*_{K,s} = \sup\limits_{\mathbf{f}}R_{K}(s, \mathbf{f}, \mathbf{g}^{*}),%\\ - \epsilon,\\
~~v^*_{K,s} = \inf\limits_{\mathbf{g}}R_{K}(s, \mathbf{f}^{*}, \mathbf{g}). $%+ \epsilon.
%\end{align*}%The 0-optimal strategies are called optimal.
\end{definition}
%\begin{remark}
%The objective of security problems is usually ensuring the performance of the "weakest" link in the system. The value of the game defined in this paper is the minimum of the worst case cost for the system, which is consistent with security goal.
%\end{remark}

%\begin{lemma}%\cite{finite_exist}
The existence conditions of the value and optimal strategies for a general finite horizon zero-sum nonstationary stochastic game are shown in~\cite{finite_exist}. The game defined in this paper has a finite state space, finite action spaces, and satisfies~\eqref{fR}.
%the state transition probability and immediate payoff functions are defined to calculate the expectation total payoff, 
%and $\sup_{\mathbf{f} \in F^{K}}R_{K}(s,\mathbf{f}, \mathbf{g}^{*})$ is bounded.
%Our game model 
%\PA{adopted?} 
Therefore, using the same approach as in the proofs from~\cite{finite_exist} we can prove the following theorem:

\begin{theorem} 
%The value of the game and an optimal strategy for each player exist for the considered problem formulation.
There exists the value of the considered game and an optimal strategy for the system.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%
%%%%%%%%%%%%%%%
\iffalse
The game we define in this paper has properties: (i) for any stage k, the state space S, action space $A_{tk}$ for attacker and $A_{sk}$ for system are finite sets.   (ii) The state transition probability matrix $\tilde{P}^{k}(s_{h}|h_{k}, s_{l})$ together with the strategy history $h_{k}$ defines a conditional distribution for computing the expected total payoff. %at stage $k+1$, given the strategy history $h_{k} \in H_{k}$ and both players' actions at stage $k$. 
(iii) The immediate payoff $\tilde{r}^{k} (h_{k},s_{l})$ is nonnegative, and conditional expected total payoff function $R_{k}(s,\mathbf{f,g}): H_{K} \to R$ is a bounded below (nonnegative), nondecreasing, for $k\in\{1,\cdots,K\}$. %lower semicontinuous function on $H_{K}$. 
%(iv)In finite time, \[\sup_{\mathbf{f} \in F^{K}}R_{K}(s,\mathbf{f}, \mathbf{g}^{*}) < \infty,s \in S.\]
The game formulation in this paper can be interpreted by the abstract nonstationary game model in~\cite{finite_exist}, and a detail proof is provided in~\cite{finite_exist}.
%%%%\end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Suboptimal Algorithm For the Nonstationary Game}

Existing value iterative algorithms for stationary stochastic games can not be used to solve our game, since the nonstationary game parameters depend on the previous history, which is only available in the future algorithm iterations.
Hence, we design a suboptimal algorithm based on the  value iteration method for finite horizon stationary stochastic game from~\cite{plangame} and robust game techniques from~\cite{RGT}. 
Algorithm~\ref{finite} provides an upper bound for the game value and the corresponding nonstationary suboptimal strategy for the system. The idea is to solve a robust game at each iteration step -- i.e., minimize the worst-case caused by extreme points of the nonstationary payoff and state transition probability polyhedra, or $(r_{k},\mathbb{P}_{k})$, defined for all possible histories. 
%Algorithm~\ref{finite} for the finite horizon nonstationary stochastic game 

%The iteration works in the way, that if a player knew how to play in the robust stochastic game optimally from the next stage on, then, at the current stage, he would play with such strategies. Similar to a stationary stochastic game, this value iteration minimizes the maximum expected immediate cost at the current stage and expected costs possibly incurred in future stages.    
 
%
%The value iteration is: %such that for given initial $v^{0}_{s}$ the value of the game at time t+1 is:
%\begin{align*}
 %                     $v^{t}_{s}=\text{value}[\tilde{r}_{s}+\sum_{s'\in S} \tilde{P}(s'|s)v^{t+1}_{s'}].$
%\end{align*}
The value iteration algorithm for finite horizon stationary stochastic game (with fixed payoff $r$ and state transition probability $P$ at every stage) works in the way that if a player knew how to play in the game optimally from the next stage on, then, at the current stage, he would play with such strategies~\cite{plangame}. The value of $K$-stage game is finally provided by the last step of iteration. Similarly, the Algorithm~\ref{finite} of the nonstationary stochastic game starts from the last stage, gets the matrix game value and the optimal strategy related to nonstationary $(r_{k},\mathbb{P}_{k})$  at each stage, and returns an upper bound for the value of the total payoff in $K$-stages. 
To estimate the values %%%%iteration of 
at each step, we consider the payoff and state transition probability set ($r_{k}$, $\mathbb{P}_{k}$) as an uncertain parameter set for the one shot robust game~\cite{RGT}. %Then approximate each iteration value as the value of the robust one shot zero sum game. 

To quantify the bounded polyhedra ($r_{k}$, $\mathbb{P}_{k}$), we need the expected system dynamics $\mathbf{x}_{k}, \mathbf{u}_{k}$, $\mathbf{y}_{k}, k=1,\cdots,K$ defined in Section~\ref{dynamicgame}, which is determined by the strategy history.  
%(this approximation also holds for other attack game quantification model with bounded payoff and transition probability). 
The extreme points for the uncertain set  ($r_{k}$, $\mathbb{P}_{k}$) depend on pure strategy histories. Let $H^p_k \subset H_k$ be the concatenation of pure strategies until stage $k$, where  a pure history $h^{p}_{k} \in H^{p}_{k}$, $h^{p}_{k}=s_{1}\mathbf{f}^{p}_{1}\mathbf{g}^{p}_{1}\cdots\mathbf{f}^{p}_{k-1}\mathbf{g}^{p}_{k-1}$ satisfies that all $f^{p}_{t}(s), g^{p}_{t}(s)$ have only one non-zero element (i.e., they choose the corresponding action or the \emph{pure} strategy).  
By using any $h^{p}_{k}$ in the game model of Section~\ref{dynamicgame}, we get the corresponding $r^p_k(h^p_k,s_l)$ and $P^p_k(h^p_k,s_l)$ for stages $1$ to $K$. Thus, the extreme points set $(r_{kp},\mathbb{P}_{kp})$ for $(r_{k}, \mathbb{P}_{k})$ is:%which we define as: \\
%\vspace{-4pt}
\begin{equation*}
\{(r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(h^{p}_{k},s_{l})) |~h^{p}_{k}\in H^{p}_{k},l\in\{1,2,3\}\}.
\end{equation*}
%\vspace{-4pt}
%%%%%%%%%%%%%%%


\iffalse
Now, consider the iteration for calculating the pure history value $v_{k}^{s_{l}}(h^{p}_{k})$ (from extreme points $(r_{kp},\mathbb{P}_{kp})$). %based on $v_{k+1}^{s'}(h^{p}_{k+1})$ of the previous inductive value iteration process at $k+1$.
We denote the non-pure history value of $k$ as $v_{k}^{s_{l}}(h^{p}_{k-1})$, which is calculated from the $(r_k,\mathbb{P}_k)$ that have pure strategies in all stages $1,\cdots,k-2$, and any strategy at stage $k-1$.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%



We define the pure strategy backup matrix set $\mathbb{Q}_{kp}$, $k=1,\cdots,K-1$ as:
%for each $(r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(h^{p}_{k},s_{l}))\in (r_{kp},\mathbb{P}_{kp})$,
\vspace{-5pt}
\footnotesize
\begin{align}
\vspace{-5pt}
\mathbb{Q}_{kp}=\{Q_{k}^{p}(h^{p}_{k},s_{l}) = r^{p}_{k}(h^{p}_{k},s_{l})+\sum_{s'\in S} P^{p}_{k}( s' |h^{p}_{k},s_{l})v_{k+1}^{s'}(h^{p}_{k+1})\},
\label{eq:Q}
\end{align}
\normalsize
where $v^{s'}_{k+1}(h^p_{k+1})\geq 0$ is the robust game value resulting from the iteration at stage $k+1$ of~Algorithm~\ref{finite}, and relates to matrix games defined by $\mathbb{Q}_{(k+1)p}$.
 In addition,  we define the backup matrix set~$\mathbb{Q}_{k}$ for all possible~$h_{k}$,  as
 
\vspace{-8pt}
\footnotesize
\begin{align*}
\vspace{-5pt}
\mathbb{Q}_{k}= 
\{&\tilde{Q}_{k}(h_{k},s_{l})=\tilde{r}_{k}(h_{k},s_{l})+\sum_{s'\in S}\tilde{P}_{k}(s'|h_{k},s_{l})v^{s'}_{k+1}(h^p_{k+1})\}.
%&h_{k} \in H_{k}, l=1,2,3\}.
\end{align*} 
\normalsize
Finally, for the stage $K$ we define $Q_{K}^{p}(h^{p}_{K},s_{l})= r^{p}_{K}(h^{p}_{K},s_{l})$ and $\tilde{Q}_{K}(h_{K},s_{l})=\tilde{r}_{K}(h_{K},s_{l})$. 

Now, consider the iteration for calculating $v_{k}^{s_{l}}(h^{p}_{k})$ from all matrix games $Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}$ in Algorithm~\ref{finite}. 
We denote the non-pure history value of $k$ as $v_{k}^{s_{l}}(h^{p}_{k-1})$, which is calculated from the $\tilde{Q}_{k}(h_{k},s_{l})$ that have the same pure strategies as $h^p_k$ in all stages $1,\cdots,k-2$, and any strategy at stage $k-1$.
We use the following result to show that  at every $k$, $v_{k}^{s_{l}}(h^{p}_{k})$ is greater than or equal to $v_{k}^{s_{l}}(h^{p}_{k-1})$.


\begin{theorem}
Consider the value iteration for stage $k$ as a one shot robust game. %given a pure strategy history $h^{p}_{k}$, 
Based on $v_{k+1}^{s'}(h^{p}_{k+1}) \geq 0$ of previous iteration, 
We define the robust game value  obtained at $k$ as %to compute $v^{k-1}_{s}(h^{p}_{k-1})$ at $k-1$ as:
\begin{align}
v^{s_{l}}_{k}(h_{k}^{p})=\max_{Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}}v^*[Q_{k}^{p}(h^{p}_{k},s_{l})],%v_{k}^{s_{l}}(h_{k}^{p})&=\max_{(r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(h^{p}_{k},s_{l}))}
%v^*[r^{p}_{k}(h^{k}_{p},s_{l})+\sum_{s'\in S} P^{p}_{k}( s' |h^{p}_{k},s_{l})v_{k+1}^{s'}(h^{p}_{k+1})],
\label{pickv}
\end{align}
where $v^*$ is the function that yields the value of a zero-sum matrix game. Then for $k=2,\cdots, K$, $v_{k}^{s_{l}}(h^{p}_{k-1})$ is upper bounded by $v_{k}^{s_{l}}(h_{k}^{p})$ (i.e.,~$v^{s_{l}}_{k}(h^{p}_{k-1})\leq v_{k}^{s_{l}}(h_{k}^{p})$).%&\max_{(r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(\cdot|h^{p}_{k},s_{l}))\in (r^{kp},\mathbb{P}^{kp})}%\in (M^{p}_{ks_{l}}(h^{p}_{k}), P^{p}_{k}( . |h^{p}_{k},s_{l}))}\\
%\text{value}[r^{p}_{k}(h^{k}_{p},s_{l})+\\
%&\sum_{s'\in S} P^{p}_{k}( s' |h^{p}_{k},s_{l})v^{k+1}_{s'}(h^{p}_{k})].
%\end{align*}
 %and we have exact 4 $v^{k+1}_{s'}(h^{p}_{k})$ for every $s' \in S$ as candidate backup value at every stage k. 
\label{robust}
\end{theorem}


\begin{proof}
%In the following proof every $h_{k}^{p}$ is a branch for the same $h^{p}_{k-1}$, $h_{k}=h_{k-1}^{p}\mathbf{f}^{k}\mathbf{g}^{k}$, and we omit the subscript $h^{p}_{k-1}$. 
\iffalse
The backup matrix set $\mathbb{Q}_{k}$ for all possible $h_{k}$ is %for $s_l$ :
\begin{align*}
%Q_{k}= 
\{&\tilde{Q}_{k}(h_{k},s_{l})=\tilde{r}_{k}(h_{k},s_{l})+\sum_{s'\in S}\tilde{P}_{k}(s'|h_{k},s_{l})v^{s'}_{k+1}(h_{k+1}^{p})\},
%&h_{k} \in H_{k}, l=1,2,3\}.
\end{align*}
\fi
%%%%%%%%%%%%%%%%%%%%%
%$\tilde{Q}_{k}\in \mathbb{Q}_k$. 
Since $v^{s'}_{k+1}(h_{k+1}^{p})$ is a nonnegative scalar, the extreme points of $\mathbb{Q}_{k}$ can only come from the extreme points of the tuple $(r_{k}, \mathbb{P}_{k})$, i.e., by considering the matrix game value of every $Q_{k}^{p} (h_{k}^{p},s_{l})$ defined in~\eqref{eq:Q}, we will get the maximum value from extreme points of $\mathbb{Q}_k$. 
%\[\tilde{Q}_{k}^{p}=\{ Q_{k}^{p} (h_{k}^{p},s_{l}), (r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(h^{p}_{k},s_{l}))\in (r^{kp},\mathbb{P}^{kp})\}.\] 
%we only need to consider every extreme point  $(r^{p}_{k}(h^{p}_{k},s_{l}), P^{p}_{k}(\cdot|h^{p}_{k},s_{l}))$ in
% 
Now consider the following optimization problem for the system~\eqref{optr} and for any attacker's strategy vector $\mathbf{f}$
%From the system's perspective, to compute the value of the matrix game is equivalent with:
\vspace{-5pt}
\begin{align}
%\begin{split}
\vspace{-5pt}
\min_{\mathbf{g}} \quad & z\label{ob_z}\\
\text{subject to}\quad &z \geq \max_{\tilde{Q}_{k}(h_{k},s_{l})\in \mathbb{Q}_{k}}\mathbf{f}^{T} [\tilde{Q}_{k}(h_{k},s_{l})]\mathbf{g}.
%\end{split}
\label{optr}
\end{align}
As proven by~Lemma 5 in \cite{RGT},~\eqref{optr} is equivalent to the following constraint that considers only the extreme points
\begin{align}
\quad z \geq \max_{Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}}\mathbf{f}^{T} [Q_{k}^{p}(h^{p}_{k},s_{l})]\mathbf{g},
\end{align}
%meaning that it is sufficient to consider only the extreme points.


For the worst-case $f$, the above is also true. Hence, let 
\begin{align}
\label{eq1}
v^{s_{l}}_{k}(h_{k}^{p})
%=\max_{Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}}v^*[Q_{k}^{p}(h^{p}_{k},s_{l})]
=\max_{Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}} \min\limits_{\mathbf{g}}\max\limits_{\mathbf{f}}\mathbf{f}^T[Q_{k}^{p}(h^{p}_{k},s_{l})]\mathbf{g}.
%\label{pickv}
\end{align}
For optimal policies $\mathbf{f}^{*}(h^{p}_{k},s_{l})$ and $\mathbf{g}^{*} (h^{p}_{k},s_{l})$, the above optimization \eqref{eq1} results in cost $\max\limits_{Q_{k}^{p}(h^{p}_{k},s_{l})\in \mathbb{Q}_{kp}}v^*[Q_{k}^{p}(h^{p}_{k},s_{l})]$. 
%we can compute the value from four different $\tilde{Q}_{ks_{l}}^{p}(h^{p}_{k})$separately, and get the value follow the pure strategy $v^{k}_{s'}(h^{p}_{k-1})$. 
However, $(\mathbf{f}^{*}(h^{p}_{k},s_{l}),\mathbf{g}^{*}(h^{p}_{k},s_{l}))$ can be non-pure strategies, meaning that when used in~\ref{dynamicgame}, they will not result in extreme points of $\mathbb{Q}_{k+1}$. The non-pure history value $v_{k+1}^{s'}(h_{k}^{p})$ of iteration for stage $k+1$ satisfies %%%%%(from $\mathbb{Q}_{(k+1)p}$):
%\begin{align*}
$
v_{k+1}^{s'}(h_{k}^{p})\leq v_{k+1}^{s'}(h_{k+1}^{p}). 
$
%\end{align*}
Replacing $v_{k+1}^{s'}(h_{k+1}^{p})$ by $v_{k+1}^{s'}(h_{k}^{p})$ in~\eqref{eq:Q} will decrease every element in matrix $Q^{p}_{k}$, since $r_{k}^{ij}\geq0$ and $P_{k}^{ij}\geq 0$. %%% by definition. 
%The system is a minimizer, and is possible to get a smaller value at time k, with some %optimal strategy history $h^{*}_{k} \neq h^{p}_{k}$, 
With a similar argument in the next iteration for stage $k-1$, we have $v_{k}^{s_{l}}(h^{p}_{k-1})\leq v^{s_{l}}_{k}(h_{k}^{p})$. 
%(Note that here $v_{k}^{s_{l}}(h^{p}_{k-1})$ is not the game value at $k$ either, because the strategies from 1 to $k-2$ must be pure to get it).
\end{proof}
%\squeezeup
%\vspace{-5pt}
\begin{algorithm}
%\vspace{-5pt}
\caption{\textbf{: Suboptimal Algorithm for A Finite Nonstationary  Stochastic Game }}
\textbf{Input}: System model parameters and game parameters.
\\\textbf{Initialization}:
             Compute the set of $(r_{kp}, \mathbb{P}_{kp})$ for $k=1,...K$.
              %For all $s_{l} \in S, l =1,2,3, h^{p}_{K}\in H^{p}_{K} :$ get %$4^{K-1}$ 
              %backup matrix set $\{Q_{k}^{p}(h_{k}^{p},s_{l})\}$:
              
             Compute the game at stage $K$: $Q_{K}^{p}(h^{p}_{K},s_{l})=r_{K}^{p}(h^{p}_{K},s_{l})$, \\ 
                    $f^{*}(h^{p}_{K}, s_{l}), g^{*}(h^{p}_{K}, s_{l}), v_{K}^{s_{l}}(h^{p}_{K}) \leftarrow \pi(Q_{K}^{p}(h^{p}_{K},s_{l}).$
\\\textbf{Iteration}: For $k=(K-1), \cdots, 1$,

get the backup matrix set $\mathbb{Q}_{kp}$ for all $h^{p}_{k}\in H^{p}_{k}$, where each matrix is defined in~\eqref{eq:Q}, then calculate:
%\[Q_{k}^{p}(h^{p}_{k},s_{l}) = r^{p}_{k}(h^{p}_{k},s_{l})+\sum_{s'\in S} P^{p}_{k}( s' |h^{p}_{k},s_{l})v_{k+1}^{s'}(h^{p}_{k+1}),\]

 $f^{*}(h^{p}_{k}, s_{l}), g^{*}(h^{p}_{k}, s_{l}),v_{k}^{s_{l}}(h^{p}_{k}) \leftarrow \pi(Q_{k}^{p}(h^{p}_{k},s_{l}))$.
 
%$\mathbf{f}^*_k=[\mathbf{f}^{*}(h^{p}_{k}, s_{l}),\mathbf{f}^{*}(h^{p}_{k}, s_{2}), \mathbf{f}^{*}(h^{p}_{k}, s_{3})],$ $ \mathbf{g}^{*}_k=[\mathbf{g}(h^{p}_{k}, s_{1}),\mathbf{g}(h^{p}_{k}, s_{2}),\mathbf{g}(h^{p}_{k}, s_{3})].$ 

$\mathbf{f}^*_k=[\mathbf{f}^{*}(h^{p}_{k}, s_{l}),l=1,2,3],$ $ \mathbf{g}^{*}_k=[\mathbf{g}^*(h^{p}_{k}, s_{l}), l=1,2,3].$ 

\textbf{Return}: the strategy concatenation pair $\mathbf{f}_{a}=\mathbf{f}^{*}_1\cdots\mathbf{f}^*_K,\mathbf{g}_{a}=\mathbf{g}^{*}_1\cdots\mathbf{g}^*_K$ and the value upper bound $v^{s_{l}}_{1},l=1,2,3$.
\label{finite}
%\vspace{-5pt}
\end{algorithm}
%\squeezeup

According to~Theorem~\ref{robust}, we use Algorithm~\ref{finite} to compute an upper bound of the value and the corresponding suboptimal strategy for every step. The % Nash Equilibrium selection 
function $\pi$ computes the strategy and robust value as defined in~\eqref{pickv}. Note that for the replay attacks considered in this paper, at state $s_{1}$ the system wins the game and replay is harmless. Thus, the optimal strategies of $s_{1}$ is $\mathbf{g}_{k}(s_{1})=\begin{bmatrix}1&0\end{bmatrix}^{T}$, $\mathbf{f}_{k}(s_{1})=\begin{bmatrix}1&0&\cdots&0\end{bmatrix}^{T}$. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%the Input can be: $\mathbf{A,B,C,Q,R,\bar{x}_{0}},\Sigma,$ $\mathbf{K},$ $\mathbf{W,U,L}$, $\tau, \alpha, \Delta \mathbf{u}_{k}\sim N(0,\mathcal{L})$; replay window size $\{t_{2},\cdots,t_{M}\}$, total stage number $K$, system initial state distribution $p(s^{1})$, false alarm trigger penalty.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The nonstationary game values $v_k^{s_l}(h^p_{k-1})$ and $v_k^{s_l}(h^p_k)$ that result from value iteration of two strategies only differ at stage $k-1$ (i.e.,~same and pure from stages 1 to $k-2$). By value iteration backward to stage 1, we compare the game value (for all possible strategies) and the robust game value $v_1^{s_l}$ of~Algorithm~\ref{finite} in the following theorem.
\begin{theorem}
%Moreover, by following this iteration method,
~Algorithm~\ref{finite} results  in an upper bound $v_{1}^{s_{l}}$ for the value of the $K$-stage game, together with suboptimal strategies $\mathbf{f}_{a}$ and $\mathbf{g}_{a}$. 
\end{theorem}
\vspace{3pt}
\begin{proof}
The strategies $\mathbf{f}_{a}, \mathbf{g}_{a}$ of~Algorithm~\ref{finite} are possibly not pure. %strategy history $h^{p}_{K} \in H^{p}_{K}$. 
According to~Theorem~\ref{robust}, $v_{k}^{s_{l}}(h^{p}_{k-1})\leq v^{s_{l}}_{k}(h_{k}^{p})$, %(may write this proof more detailed depends on the paper requirement)
and the proof holds for every $k=2,\cdots,K$.  \iffalse Using induction,\fi Consider the value iteration for $k=1$, with $v_{2}^{s_{l}}(h^{p}_{1})\leq v^{s_{l}}_{2}(h_{2}^{p})$, 
\footnotesize
\begin{equation*}
\vspace{-5pt}
Q_1^{ij}(h_1, s_l)=\tilde{r}_1^{ij}(h_1,s_l)+\sum\limits_{s'\in S}\tilde{P}^{ij}_{1}(s'|h_{1},s_{l})v^{s'}_{2}(h^p_{1})\leq Q_1^{ij}(h_2^p,s_l),
\end{equation*}
\normalsize
thus $v^{*}[Q_1(h_1, s_l)] \leq v^{s_{l}}_{1}$.  Iterative value based on pure strategy back up matrix sets $\mathbb{Q}_{kp}, k=1,\cdots, K$ obtained from~Algorithm~\ref{finite} is an upper bound for the game value.
\end{proof}

\iffalse
\begin{remark} %%%%%\FM{remove this remark to the extension paper?}
Algorithm~\ref{finite} is exponential with K, and for large control system running time $\tilde{T}$, the game stage $K$ does not need to be $\tilde{T}$--% We can formulate a $K$-stage game, 
each stage we compute $\tilde{T}/K$ steps of control system dynamic, and apply the average cost and transition probability to quantify the game parameters. 
%keeps the same during each stage ($\tilde{T}/K$ time).  
In particular, if we consider the infinite horizon problem, the game formulation can reduce to stationary. 
For example, we can define the infinite time average LQG cost as the payoff function, and the average detection rate/false alarm trigger rate as state transition probability, and find the optimal strategy of a stationary stochastic game.
%Or assume the replay window size does not change during K.
\end{remark}%\FM{we can put this remark at the end of section 3?}
\fi
